ThinK: Thinner Key Cache by Query-Driven Pruning

Large Language Models (LLMs) have revolutionized the field of natural language processing, achieving unprecedented performance across a variety of applications. However, their increased computational and memory demands present significant challenges, especially when handling long sequences. This paper focuses on the long-context scenario, addressing the inefficiencies in KV cache memory consumption during inference. Unlike existing approaches that optimize the memory based on the sequence length, we identify substantial redundancy in the channel dimension of the KV cache, as indicated by an uneven magnitude distribution and a low-rank structure in the attention weights. In response, we propose ThinK, a novel query-dependent KV cache pruning method designed to minimize attention weight loss while selectively pruning the least significant channels. Our approach not only maintains or enhances model accuracy but also achieves a reduction in KV cache memory costs by over 20% compared with vanilla KV cache eviction and quantization methods. For instance, ThinK integrated with KIVI can achieve a 2.8x reduction in peak memory usage while maintaining nearly the same quality, enabling up to a 5x increase in batch size when using a single GPU. Extensive evaluations on the LLaMA and Mistral models across various long-sequence datasets verified the efficiency of ThinK, establishing a new baseline algorithm for efficient LLM deployment without compromising performance. Our code has been made available at https://github.com/SalesforceAIResearch/ThinK.

==> myheaders.tex <==
%\usepackage{fullpage}


%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


\newcommand{\hanze}[1]{{\textcolor{orange}{[Hanze: #1]} }}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{Equation~(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
%-----------------------------------------------------------------%
%
% Han Zhong: This style file is modified by the latex macro of the 
% SMiLe group (Han Liu).                  
%
%-----------------------------------------------------------------%
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage{bm} 
\RequirePackage{url}
\usepackage{multirow}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{array}
\usepackage{url}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{dsfont}


% -------- New Packages -------- %
\usepackage{enumitem}

%------ kpfonts -------%
%\usepackage{kpfonts}

%------- some other packages -------%
\usepackage{enumerate}
\usepackage[OT1]{fontenc}
\usepackage{natbib}




\usepackage{mathrsfs}


\usepackage{xcolor}
\usepackage{hyperref}

\iffalse
\usepackage[dvipsnames, svgnames, x11names]{xcolor}
\usepackage[colorlinks,
            linkcolor=RoyalBlue,
            anchorcolor=RoyalBlue,
            citecolor=RoyalBlue
            ]{hyperref}

%\usepackage[dvipsnames, svgnames, x11names]{xcolor}
\usepackage[colorlinks,
            linkcolor=RoyalBlue,
            anchorcolor=RoyalBlue,
            citecolor=RoyalBlue
            ]{hyperref}
\fi


%------- new defines -------%


\def\##1\#{\begin{align}#1\end{align}}
\def\$#1\${\begin{align*}#1\end{align*}}


%\let\hat\widehat
\let\tilde\widetilde
\let\check\widecheck
\def\given{{\,|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}


\def\TV{\mathrm{TV}}
%----- bold fonts -----%

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}
\newcommand{\bftau}{\mathbf{\tau}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}




%----- blackboard bold fonts-----%
\newcommand{\AAA}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\OOmega}{\mathbb{\Omega}}

\newcommand{\reg}{\mathrm{Reg}}

\usepackage{xcolor}

\definecolor{red1}{HTML}{f47983}
\definecolor{blue1}{HTML}{3eede7}
\definecolor{yellow1}{HTML}{f5dd6f}
%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


%----- Some standard definitions -----%

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}


\DeclareMathOperator{\Cor}{\rm Corr}

\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}  
                                                        
\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}

%%%%%% Complexity
\newcommand{\dca}{{\mathrm{DC}}}
\newcommand{\ec}{{\mathrm{EC}}}
\newcommand{\de}{{\mathrm{dim_{DE}}}}
\newcommand{\bde}{{\mathrm{dim_{BE}}}}
\newcommand{\dotprod}[1]{\left\langle #1\right\rangle}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms

\newcommand{\norm}[1]{\|#1\|}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\off}{\mathrm{off}}

\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\mle}{\mathrm{MLE}}

\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\hpi}{\hat \pi}
\newcommand{\hnu}{\hat \nu}
\newcommand{\hmu}{\hat \mu}
\newcommand{\hM}{\widehat{M}}
\newcommand{\hcM}{\widehat{\cM}}
\newcommand{\DG}{\mathrm{DuaGP}}
\newcommand{\tool}{\mathrm{tool}}
\newcommand{\hcP}{\widehat{\cP}}
\newcommand{\hR}{\hat{R}}
\newcommand{\hP}{\hat{P}}
\newcommand{\tGamma}{\tilde{\Gamma}}
\newcommand{\tv}{\mathrm{TV}}

\newcommand{\bra}[1]{\left[#1\right]}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\tpi}{\tilde{\pi}}
\newcommand{\epsr}{\varepsilon_{r}}
\newcommand{\piso}{\pi_{t^*}^1}
\newcommand{\tg}{\widetilde \Gamma}
\newcommand{\inner}[1]{ \left\langle {#1} \right\rangle }
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Reg}{\mathfrak{R}}
\newcommand{\joff}{\hat{J}_{\mathrm{off}}}

==> tables/kv-pruning.tex <==
\begin{table}[htp]
    \centering \scriptsize
    \caption{Performance comparison of pruning both K and V cache with different pruning ratios on LongBench.}\vspace{4pt}\label{tab:pruningkv}
\scalebox{0.6}{\begin{tabular}{l|lcccccccccccccccccc}
    \toprule
&\multirow{4}{*}{Method}& \multirow{4}{*}{$\gamma$}& \multicolumn{3}{c}{Single-Document QA} & \multicolumn{3}{c}{Multi-Document QA}& \multicolumn{3}{c}{Summarization}& \multicolumn{3}{c}{Few-shot Learning}& \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{Code}&\multirow{4}{*}{Avg.} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}
&&& \rotatebox[origin=c]{30}{NrtvQA} & \rotatebox[origin=c]{30}{Qasper} & \rotatebox[origin=c]{30}{MF-en} & \rotatebox[origin=c]{30}{HotpotQA} & \rotatebox[origin=c]{30}{2WikiMQA} & \rotatebox[origin=c]{30}{Musique} & \rotatebox[origin=c]{30}{GovReport} & \rotatebox[origin=c]{30}{QMSum} & \rotatebox[origin=c]{30}{MultiNews} & \rotatebox[origin=c]{30}{TREC} & \rotatebox[origin=c]{30}{TriviaQA} & \rotatebox[origin=c]{30}{SAMSum} & \rotatebox[origin=c]{30}{PCount} & \rotatebox[origin=c]{30}{PRe} & \rotatebox[origin=c]{30}{Lcc} & \rotatebox[origin=c]{30}{RB-P} \\
&\multicolumn{19}{c}{KV-size Full}\\
\multirow{28}{*}{\rotatebox[origin=c]{90}{ LLaMA3 8B}}

    & ALL KV & 0  & 25.56 & 32.27 & 39.71 & 43.56 & 35.09 & 21.18 & 28.71 & 23.26 & 26.64 & 73.5 & 90.48 & 42.33 & 4.8 & 69.25 & 59.29 & 54.05 & 41.86 \\
\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 128}\\
    & H2O         & 0   & 22.12 & 13.20 & 31.61 & 37.79 & 32.71 & 18.45 & 20.32 & 22.02 & 21.10 & 38.50 & 87.75 & 39.14 & 5.83 & 69.50 & 55.06 & 50.97 & 35.38 \\
    & H2O(99)     & 0   & 21.13 & 12.01 & 29.34 & 37.30 & 30.51 & 18.64 & 19.41 & 21.80 & 20.65 & 38.50 & 86.97 & 38.37 & 5.60 & 69.00 & 55.13 & 51.46 & 34.74 \\
    & H2O+\our(l1)    & 20+40  & 23.04 & 12.94 & 31.36 & 42.17 & 33.49 & 18.74 & 19.13 & 21.99 & 20.40 & 37.50 & 85.39 & 37.71 & 5.84 & 67.77 & 54.84 & 52.31 & 35.29 \\
    & H2O+\our(l2)    & 20+40  & 23.35 & 13.42 & 31.24 & 42.67 & 34.89 & 18.98 & 19.28 & 21.65 & 20.11 & 37.50 & 84.46 & 37.32 & 6.15 & 68.42 & 54.72 & 51.33 & 35.34 \\
    & H2O+\our(new)    & 30+30  & 22.72 & 13.88 & 31.47 & 41.68 & 31.86 & 19.1 & 19.85 & 21.98 & 20.48 & 38.00 & 84.79 & 37.99 & 6.10 & 69.50 & 57.83 & 55.38 & 35.79 \\
    & H2O+\our(new2)    & 30+30  & 23.71 & 13.65 & 33.08 & 41.86 & 29.88 & 18.04 & 19.60 & 21.65 & 20.26 & 38.00 & 86.08 & 38.61 & 5.16 & 69.50 & 57.59 & 55.19 & 35.74 \\
    & H2O+\our(new2)    & 40+0  & 22.85 & 14.55 & 29.49 & 38.63 & 30.84 & 18.90 & 20.12 & 21.96 & 20.68 & 38.50 & 86.38 & 38.40 & 5.50 & 69.17 & 57.93 & 56.12 & 35.63 \\
    & H2O+\our(new2)    & 50+0  & 23.47 & 14.06 & 28.67 & 38.35 & 30.21 & 17.87 & 19.69 & 21.94 & 19.95 & 38.50 & 87.14 & 38.07 & 4.92 & 69.50 & 57.99 & 56.66 & 35.44 \\
    \cdashline{2-20}    
    & SnapKV      & 0  & 21.19 & 13.55 & 32.64 & 38.75 & 29.64 & 18.73 & 18.98 & 21.62 & 20.26 & 45.00 & 88.36 & 37.64 & 5.13 & 68.85 & 55.84 & 51.82 & 35.50 \\
    & SnapKV(99)  & 0  & 20.37 & 11.51 & 33.94 & 37.78 & 28.79 & 19.37 & 17.85 & 21.46 & 19.22 & 42.00 & 87.52 & 37.83 & 5.42 & 68.83 & 54.97 & 51.11 & 34.87 \\
    & SnapKV+\our(l1) & 20+40 & 22.22 & 14.35 & 36.13 & 43.55 & 32.55 & 19.51 & 18.36 & 21.20 & 19.08 & 41.00 & 86.82 & 36.99 & 6.07 & 69.50 & 56.18 & 51.18 & 35.92 \\
    & SnapKV+\our(l2) & 20+40 & 22.96 & 14.54 & 34.81 & 43.81 & 31.66 & 19.44 & 18.34 & 21.31 & 18.84 & 41.50 & 86.82 & 37.17 & 6.07 & 69.50 & 55.87 & 52.03 & 35.92 \\
    & SnapKV+\our(new) & 30+30 & 22.75 & 15.27 & 33.68 & 42.89 & 31.24 & 19.15 & 19.00 & 20.72 & 19.51 & 42.00 & 87.64 & 37.41 & 6.07 & 68.98 & 58.24 & 56.32 & 36.30 \\
    & SnapKV+\our(new2)& 30+30  & 21.86 & 13.79 & 33.26 & 40.93 & 29.39 & 19.22 & 18.81 & 21.30 & 19.26 & 41.50 & 87.00 & 37.95 & 5.78 & 69.50 & 57.84 & 55.62 & 35.81 \\
    & SnapKV+\our(new2)& 40+0  & 22.11 & 14.67 & 32.49 & 36.25 & 28.63 & 18.80 & 18.93 & 21.49 & 20.14 & 44.50 & 88.11 & 38.32 & 5.75 & 69.17 & 58.21 & 55.89 & 35.84 \\
    & SnapKV+\our(new2)& 50+0  & 21.79 & 14.73 & 32.03 & 37.52 & 27.86 & 18.28 & 18.50 & 21.52 & 19.71 & 43.50 & 86.00 & 38.35 & 5.59 & 69.50 & 57.96 & 56.96 & 35.61 \\

    % & PyramidKV   & 0 & 21.40 & 16.92 & 33.79 & 39.73 & 28.72 & 18.59 & 19.86 & 22.48 & 20.95 & 66.50 & 89.35 & 38.39 & 5.92 & 69.00 & 56.49 & 47.95 & 37.25 \\
    % & PyramidKV(99)& 0 & 21.27 & 15.39 & 32.12 & 40.40 & 27.47 & 19.69 & 19.56 & 22.28 & 20.58 & 63.00 & 87.94 & 38.54 & 5.92 & 68.79 & 55.48 & 47.64 & 36.63 \\
    % & PyramidKV+\our & 20+40 & 21.65 & 18.96 & 32.97 & 40.50 & 27.99 & 19.70 & 19.72 & 21.74 & 20.78 & 64.50 & 89.04 & 36.84 & 5.91 & 69.50 & 54.88 & 47.39 & 37.00\\
\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 512}\\
    & H2O         & 0   & 23.52 & 17.93 & 34.68 & 42.11 & 33.52 & 19.92 & 22.11 & 22.56 & 23.82 & 41.00 & 90.46 & 40.20 & 5.87 & 69.50 & 56.71 & 51.69 & 37.23 \\
    & H2O(400)    & 0   & 23.03 & 16.74 & 32.61 & 41.79 & 31.65 & 19.51 & 21.47 & 22.45 & 23.46 & 40.50 & 90.59 & 40.08 & 5.55 & 69.50 & 57.28 & 50.80 & 36.69 \\
    & H2O+\our(l1)    & 20+40  & 22.43 & 17.37 & 35.84 & 41.76 & 34.28 & 21.61 & 20.93 & 22.01 & 22.81 & 38.50 & 90.01 & 38.80 & 5.87 & 69.50 & 57.57 & 52.22 & 36.97 \\
    & H2O+\our(l2)    & 20+40  & 22.46 & 18.05 & 35.61 & 42.13 & 35.27 & 22.04 & 20.93 & 21.90 & 22.66 & 38.50 & 88.98 & 38.59 & 5.79 & 69.50 & 58.29 & 52.78 & 37.09 \\
    & H2O+\our(new)    & 20+40  & 22.08 & 18.35 & 35.03 & 40.99 & 34.69 & 21.31 & 20.91 & 22.02 & 22.86 & 38.50 & 89.07 & 39.42 & 5.6 & 69.5 & 59.83 & 57.04 & 37.33 \\
    & H2O+\our(new)    & 30+30  & 24.10 & 18.50 & 33.10 & 41.23 & 33.75 & 20.05 & 21.68 & 22.04 & 23.09 & 38.50 & 89.78 & 39.79 & 5.76 & 69.5 & 59.58 & 56.93  & 37.34 \\
    & H2O+\our(new2)    & 30+30  & 22.83 & 17.57 & 34.18 & 42.67 & 33.52 & 19.95 & 21.17 & 22.23 & 22.82 & 38.5 & 90.11 & 39.08 & 5.21 & 69.0 & 59.99 & 56.83 & 37.23 \\
    & H2O+\our(new2)    & 40+0  & 23.70 & 17.76 & 33.81 & 40.39 & 30.75 & 19.00 & 21.82 & 22.47 & 23.59 & 41.0 & 90.16 & 40.52 & 5.71 & 69.50 & 60.86 & 57.46 & 37.41 \\
    & H2O+\our(new2)    & 50+0  & 24.03 & 17.02 & 34.91 & 40.03 & 30.40 & 19.12 & 21.63 & 22.7 & 23.27 & 41.0 & 90.46 & 40.53 & 5.23 & 69.33 & 60.49 & 58.16 & 37.39 \\
    \cdashline{2-20}    
    & SnapKV      & 0  & 24.84 & 23.96 & 38.77 & 42.75 & 34.55 & 20.87 & 22.26 & 22.61 & 23.97 & 70.00 & 90.52 & 40.29 & 5.81 & 69.50 & 59.04 & 51.81 & 40.10 \\
    & SnapKV(400) & 0  & 25.26 & 22.73 & 37.21 & 42.86 & 33.20 & 21.74 & 22.23 & 22.27 & 23.36 & 68.00 & 90.52 & 40.35 & 5.56 & 69.50 & 59.09 & 52.44 & 39.77 \\
    & SnapKV+\our(l1) & 20+40 & 23.95 & 25.89 & 37.98 & 44.41 & 36.84 & 21.49 & 20.69 & 22.53 & 23.07 & 65.50 & 90.06 & 38.70 & 5.94 & 69.50 & 59.66 & 54.34 & 40.03 \\
    & SnapKV+\our(l2) & 20+40 & 23.77 & 25.61 & 39.05 & 44.68 & 36.24 & 21.55 & 20.59 & 22.54 & 23.06 & 66.50 & 90.36 & 38.83 & 5.83 & 69.50 & 59.10 & 54.65 & 40.12 \\
    & SnapKV+\our(new) & 20+40 & 23.58 & 26.62 & 37.32 & 45.14 & 36.94 & 21.85 & 21.16 & 22.13 & 23.11 & 66.00 & 90.44 & 39.32 & 6.08 & 69.50 & 60.84 & 57.56 & 40.47 \\
    & SnapKV+\our(new) & 30+30 & 23.86 & 25.88 & 36.67 & 44.17 & 36.12 & 21.45 & 21.40 & 22.5 & 23.89 & 67.00 & 90.39 & 40.03 & 6.04 & 69.5 & 61.28 & 58.24 & 40.53 \\
    & SnapKV+\our(new2) & 30+30 & 24.57 & 24.59 & 38.09 & 44.61 & 34.37 & 20.37 & 21.23 & 21.95 & 23.3 & 66.00 & 90.69 & 39.38 & 5.6 & 69.00 & 61.75 & 58.46 & 40.25 \\
    & SnapKV+\our(new2) & 40+0 & 24.71 & 25.01 & 36.9 & 41.67 & 33.52 & 20.1 & 22.07 & 22.51 & 24.4 & 69.5 & 90.39 & 40.55 & 6.06 & 69.5 & 62.11 & 59.48 & 40.53 \\
    & SnapKV+\our(new2) & 50+0 & 24.79 & 24.71 & 37.34 & 41.75 & 31.52 & 20.6 & 21.92 & 22.49 & 24.09 & 69.0 & 90.39 & 40.32 & 5.79 & 69.81 & 61.58 & 59.44 & 40.35 \\

    % & PyramidKV+\our & 20+40 & 24.07 & 26.38 & 39.60 & 44.45 & 32.68 & 21.66 & 21.87 & 22.34 & 23.88 & 71.5 & 90.64 & 39.07 & 5.83 & 69.50 & 56.66 & 48.69 & 39.93 \\
\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 2048}\\
    & H2O         & 0   & 25.56 & 26.85 & 39.54 & 44.30 & 32.92 & 21.09 & 24.68 & 23.01 & 26.16 & 53.00 & 90.65 & 41.84 & 4.91 & 69.25 & 58.43 & 51.31 & 39.59 \\
    & H2O(1480)   & 0   & 25.36 & 24.42 & 39.36 & 42.62 & 34.67 & 20.42 & 23.82 & 22.78 & 25.81 & 49.50 & 90.61 & 41.81 & 5.51 & 69.25 & 58.51 & 51.10 & 39.10 \\
    & H2O+\our(l1)    & 20+40  & 24.32 & 26.25 & 39.87 & 44.80 & 34.55 & 20.74 & 21.94 & 22.88 & 25.16 & 46.50 & 90.59 & 39.91 & 6.04 & 69.50 & 60.54 & 54.44 & 39.25 \\
    & H2O+\our(l2)    & 20+40  & 23.55 & 26.55 & 40.94 & 44.84 & 35.19 & 21.10 & 22.44 & 22.44 & 24.55 & 49.00 & 90.67 & 40.19 & 6.04 & 69.50 & 60.46 & 54.27 & 39.48 \\
    & H2O+\our(new)    & 30+30  & 24.75 & 25.84 & 39.23 & 43.92 & 34.06 & 21.10 & 22.59 & 22.67 & 25.40 & 50.00 & 90.73 & 40.80 & 6.08 & 69.25 & 61.28 & 57.71 & 39.71 \\
    & H2O+\our(new2)    & 30+30  & 25.03 & 26.77 & 39.68 & 42.12 & 33.08 & 19.59 & 23.00 & 22.89 & 25.27 & 51.00 & 91.11 & 40.58 & 5.23 & 69.00 & 61.12 & 57.95 & 39.59 \\
    & H2O+\our(new2)    & 40+40  & 24.87 & 24.31 & 37.77 & 43.13 & 34.42 & 19.60 & 21.67 & 22.7 & 24.52 & 49.00 & 90.81 & 39.28 & 6.00 & 69.00 & 61.81 & 58.08 & 39.19 \\
    & H2O+\our(new2)    & 40+0  &25.56 & 26.14 & 39.26 & 42.96 & 31.52 & 20.53 & 24.43 & 23.3 & 26.07 & 53.5 & 90.56 & 41.39 & 5.52 & 69.5 & 61.93 & 58.99 & 40.07 \\
    & H2O+\our(new2)    & 50+0 & 25.01 & 25.58 & 38.97 & 42.2 & 31.68 & 20.46 & 23.94 & 23.32 & 25.95 & 53.0 & 90.37 & 40.95 & 5.13 & 69.5 & 62.26 & 58.83 & 39.82 \\
    & H2O+\our(new2)    & 60+0  & 24.26 & 22.68 & 38.43 & 40.30 & 30.10 & 20.32 & 22.37 & 22.90 & 24.98 & 50.00 & 90.16 & 39.89 & 5.39 & 69.50 & 60.15 & 58.90 & 38.77 \\
    
    \cdashline{2-20}    
    & SnapKV      & 0  & 25.86 & 29.55 & 41.10 & 44.99 & 35.80 & 21.81 & 25.98 & 23.40 & 26.46 & 73.50 & 90.56 & 41.66 & 5.17 & 69.25 & 58.67 & 51.52 & 41.58 \\
    & SnapKV(1480)& 0  & 25.75 & 28.79 & 41.01 & 45.15 & 35.43 & 21.12 & 25.13 & 22.93 & 26.01 & 72.50 & 90.56 & 41.37 & 5.23 & 69.25 & 59.11 & 51.81 & 41.32 \\
    & SnapKV+\our(l1) & 20+40 & 24.75 & 30.80 & 40.20 & 45.74 & 35.66 & 22.07 & 22.77 & 23.08 & 24.95 & 72.00 & 90.09 & 39.22 & 6.00 & 69.00 & 60.34 & 54.19 & 41.30 \\
    & SnapKV+\our(l2) & 20+40 & 24.21 & 30.47 & 40.76 & 45.30 & 35.08 & 22.37 & 22.50 & 22.93 & 24.90 & 72.00 & 90.14 & 39.26 & 6.00 & 69.25 & 60.70 & 54.74 & 41.30 \\
    & SnapKV+\our(new) & 30+30 & 24.18 & 30.63 & 38.42 & 44.28 & 34.81 & 21.83 & 23.52 & 22.71 & 25.40 & 72.50 & 90.18 & 40.79 & 5.83 & 69.25 & 61.17 & 58.42 & 41.49 \\
    & SnapKV+\our(new2) & 30+30 & 25.13 & 29.97 & 40.35 & 44.12 & 34.64 & 19.94 & 23.62 & 23.03 & 25.30 & 72.50 & 90.78 & 39.46 & 5.35 & 69.00 & 61.50 & 57.91 & 41.41 \\
    & SnapKV+\our(new2) & 40+40 & 25.13 & 28.85 & 40.7 & 44.21 & 36.36 & 21.07 & 22.31 & 22.89 & 24.80 & 72.5 & 90.88 & 38.77 & 6.41 & 69.00 & 61.49 & 58.87 & 41.52 \\
    & SnapKV+\our(new2) & 40+0 & 25.38 & 29.86 & 39.2 & 43.35 & 33.74 & 21.49 & 25.76 & 23.06 & 26.59 & 73.0 & 90.56 & 42.04 & 5.81 & 69.5 & 62.37 & 59.33 & 41.94 \\
    & SnapKV+\our(new2) & 50+0 & 25.01 & 30.0 & 39.33 & 43.24 & 33.36 & 20.77 & 25.26 & 23.41 & 26.48 & 73.0 & 90.37 & 41.44 & 5.45 & 69.5 & 62.53 & 59.79 & 41.81 \\
    & SnapKV+\our(new2) & 60+0 & 24.83 & 29.26 & 40.42 & 41.4 & 30.42 & 21.34 & 23.73 & 22.97 & 25.29 & 72.50 & 90.36 & 38.46 & 5.71 & 69.50 & 60.57 & 59.59 & 41.02 \\
    % & PyramidKV & 0 & 25.32 & 29.70 & 41.02 & 44.99 & 35.93 & 22.41 & 26.97 & 23.67 & 26.21 & 73.5 & 90.56 & 41.74 & 4.71 & 69.50 & 58.77 & 50.83 & 41.61 \\
    % & PyramidKV(1480)& 0 & 25.52 & 29.22 & 39.90 & 45.37 & 35.21 & 21.91 & 25.82 & 23.37 & 26.22 & 72.50 & 90.56 & 41.86 & 5.64 & 69.50 & 58.73 & 51.86 & 41.45 \\
    % & PyramidKV+\our & 20+40 & 25.32 & 29.70 & 41.02 & 44.99 & 35.93 & 22.41 & 26.97 & 23.67 & 26.21 & 73.50 & 90.56 & 41.74 & 4.71 & 69.50 & 58.77 & 50.83 & 41.61 \\
    
    
    %& - & 44.8 & 35.7 & \textcolor{red}{3537 chars} & 69.3 & 39.0 & 58.2\\
    %Ours-Mix2 & 0.001 & 41.9  & 22.1 & 382 & 78.8 & 66.5 & 62.4 \\
    %Ours-Mix2 & No & 37.2  & 29.1 & 656 & - & 64.6 & 60.8\\
%     \midrule
% &\multicolumn{19}{c}{KV-size 512}\\
%     & H2O         & 0   &  21.83 & 26.49 & 45.02 & 34.63 & 23.17 & 15.08 & 20.98 & 23.06 & 4.53 & 42.00 & 85.22 & 41.49 & 5.50 & 89.25 & 49.84 & 45.38 & 35.84 \\
%     & H2O(400)    & 0   &  21.93 & 24.63 & 43.55 & 33.14 & 23.37 & 14.49 & 20.85 & 23.26 & 4.40 & 41.00 & 84.46 & 41.02 & 5.50 & 88.75 & 49.28 & 45.05 & 35.29 \\
%     & H2O+\our    & 20+40  & 22.50 & 24.00 & 43.20 & 34.58 & 23.83 & 14.75 & 19.36 & 22.79 & 4.15 & 40.00 & 85.92 & 40.42 & 5.00 & 69.67 & 48.81 & 44.29 & 33.95 \\
    
%     & SnapKV      & 0  & 24.51 & 27.81 & 48.90 & 40.76 & 25.46 & 17.34 & 21.64 & 22.96 & 4.65 & 67.00 & 85.88 & 41.26 & 5.56 & 88.4 & 50.8 & 47.55 & 38.78 \\
%     & SnapKV(400) & 0  & 23.48 & 26.57 & 48.83 & 40.17 & 24.07 & 16.86 & 21.17 & 23.13 & 4.44 & 66.00 & 85.69 & 41.11 & 5.50 & 89.94 & 50.36 & 47.34 & 38.42 \\
%     & SnapKV+\our & 20+40 & 25.65 & 26.34 & 47.71 & 40.10 & 25.31 & 16.42 & 19.48 & 22.93 & 4.45 & 63.50 & 86.75 & 39.82 & 5.00 & 72.50 & 50.11 & 46.46 & 37.03 \\  
%     & SnapKV      & 0  & 24.51 & 27.81 & 48.90 & 40.76 & 25.46 & 17.34 & 21.64 & 22.96 & 4.65 & 67.00 & 85.88 & 41.26 & 5.56 & 88.4 & 50.8 & 47.55 & 38.78 \\
%     & SnapKV(400) & 0  & 23.48 & 26.57 & 48.83 & 40.17 & 24.07 & 16.86 & 21.17 & 23.13 & 4.44 & 66.00 & 85.69 & 41.11 & 5.50 & 89.94 & 50.36 & 47.34 & 38.42 \\
%     & SnapKV+\our & 20+40 & 25.65 & 26.34 & 47.71 & 40.10 & 25.31 & 16.42 & 19.48 & 22.93 & 4.45 & 63.50 & 86.75 & 39.82 & 5.00 & 72.50 & 50.11 & 46.46 & 37.03 \\
    \bottomrule
    \end{tabular}}
    \end{table}



==> tables/kv-ratio.tex <==
\begin{table}[htp]
    \centering \scriptsize
    \caption{Comparison of Pruning Ratios for K and V on LongBench.}\vspace{4pt}\label{tab:pruningratio}
\scalebox{0.6}{\begin{tabular}{l|lcccccccccccccccccc}
    \toprule
&\multirow{4}{*}{~~~Method}& \multirow{4}{*}{$\gamma$}& \multicolumn{3}{c}{Single-Document QA} & \multicolumn{3}{c}{Multi-Document QA}& \multicolumn{3}{c}{Summarization}& \multicolumn{3}{c}{Few-shot Learning}& \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{Code}&\multirow{4}{*}{Avg.} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}
&&& \rotatebox[origin=c]{30}{NrtvQA} & \rotatebox[origin=c]{30}{Qasper} & \rotatebox[origin=c]{30}{MF-en} & \rotatebox[origin=c]{30}{HotpotQA} & \rotatebox[origin=c]{30}{2WikiMQA} & \rotatebox[origin=c]{30}{Musique} & \rotatebox[origin=c]{30}{GovReport} & \rotatebox[origin=c]{30}{QMSum} & \rotatebox[origin=c]{30}{MultiNews} & \rotatebox[origin=c]{30}{TREC} & \rotatebox[origin=c]{30}{TriviaQA} & \rotatebox[origin=c]{30}{SAMSum} & \rotatebox[origin=c]{30}{PCount} & \rotatebox[origin=c]{30}{PRe} & \rotatebox[origin=c]{30}{Lcc} & \rotatebox[origin=c]{30}{RB-P} \\
\multirow{9}{*}{\rotatebox[origin=c]{90}{ LLaMA3 8B}}

    & ALL KV & 0  &25.70 &29.75 &41.12 &45.55 &35.87 &22.35 &25.63 &23.03 &26.21 &73.00 &90.56 &41.88 &4.67 &69.25 &58.05 &50.77 &41.46 \\
\cmidrule{2-20}
    & H2O         & 0   & 23.52 & 17.93 & 34.68 & 42.11 & 33.52 & 19.92 & 22.11 & 22.56 & 23.82 & 41.00 & 90.46 & 40.20 & 5.87 & 69.50 & 56.71 & 51.69 & 37.23 \\
    & H2O+\our    & 30+30  & 22.96 & 16.95 & 36.20 & 41.70 & 33.49 & 20.55 & 20.74 & 22.02 & 23.07 & 38.00 & 89.96 & 40.16 & 6.08 & 69.17 & 57.11 & 53.59 & 36.98 \\
    & H2O+\our    & 40+40  & 22.94 & 15.21 & 33.20 & 43.12 & 34.40 & 21.22 & 19.92 & 22.18 & 21.89 & 37.50 & 88.64 & 37.28 & 6.19 & 69.50 & 57.09 & 52.58 & 36.43\\
    & H2O+\our    & 20+40  & 22.43 & 17.37 & 35.84 & 41.76 & 34.28 & 21.61 & 20.93 & 22.01 & 22.81 & 38.50 & 90.01 & 38.80 & 5.87 & 69.50 & 57.57 & 52.22 & 36.97 \\
    & H2O+\our    & 30+40  & 22.36 & 17.56 & 35.05 & 42.45 & 33.76 & 21.00 & 20.35 & 21.72 & 22.56 & 38.00 & 89.54 & 38.25 & 5.81 & 69.17 & 58.15 & 52.38 & 36.76 \\
    & H2O+\our    & 30+50  & 22.84 & 16.62 & 34.99 & 43.06 & 33.12 & 21.23 & 19.84 & 22.05 & 21.74 & 37.50 & 90.08 & 37.51 & 5.83 & 69.17 & 57.04 & 51.37 & 36.50 \\
    & H2O+\our    & 20+60  & 23.19 & 17.09 & 34.15 & 43.30 & 34.47 & 21.17 & 19.78 & 22.21 & 21.39 & 37.00 & 90.13 & 37.46 & 6.08 & 69.50 & 56.09 & 51.32 & 36.52 \\

\cmidrule{2-20}
    & SnapKV      & 0  & 24.84 & 23.96 & 38.77 & 42.75 & 34.55 & 20.87 & 22.26 & 22.61 & 23.97 & 70.00 & 90.52 & 40.29 & 5.81 & 69.50 & 59.04 & 51.81 & 40.10 \\
    & SnapKV+\our & 30+30 & 24.66 & 24.92 & 38.10 & 44.57 & 35.81 & 21.29 & 20.59 & 22.51 & 22.88 & 59.00 & 90.23 & 38.55 & 5.75 & 68.05 & 59.62 & 54.68 & 39.45 \\
    & SnapKV+\our & 40+40 & 24.66 & 23.76 & 36.87 & 44.86 & 36.88 & 20.90 & 20.00 & 22.50 & 22.45 & 50.00 & 89.61 & 38.11 & 6.14 & 69.50 & 58.31 & 54.87 & 38.71 \\
    & SnapKV+\our & 20+40 & 23.95 & 25.89 & 37.98 & 44.41 & 36.84 & 21.49 & 20.69 & 22.53 & 23.07 & 65.50 & 90.06 & 38.70 & 5.94 & 69.50 & 59.66 & 54.34 & 40.03 \\
    & SnapKV+\our & 30+40 & 24.66 & 24.92 & 38.10 & 44.57 & 35.81 & 21.29 & 20.59 & 22.51 & 22.88 & 59.00 & 90.23 & 38.55 & 5.75 & 68.05 & 59.62 & 54.68 & 39.45 \\
    & SnapKV+\our & 30+50 & 23.99 & 23.27 & 37.32 & 45.11 & 35.17 & 22.15 & 19.85 & 21.83 & 22.62 & 57.00 & 90.76 & 37.67 & 5.98 & 68.70 & 58.27 & 54.18 & 38.99 \\
    & SnapKV+\our & 20+60 & 22.22 & 23.82 & 36.54 & 44.97 & 36.24 & 21.24 & 20.22 & 22.09 & 22.03 & 60.50 & 90.33 & 37.09 & 6.21 & 69.50 & 57.86 & 53.30 & 39.01 \\
    %& - & 44.8 & 35.7 & \textcolor{red}{3537 chars} & 69.3 & 39.0 & 58.2\\
    %Ours-Mix2 & 0.001 & 41.9  & 22.1 & 382 & 78.8 & 66.5 & 62.4 \\
    %Ours-Mix2 & No & 37.2  & 29.1 & 656 & - & 64.6 & 60.8\\
    \bottomrule
    \end{tabular}}
    \end{table}


==> tables/mistral.tex <==
\begin{table}[htp]
    \centering \scriptsize
    \caption{Performance comparison of pruning both K cache with different pruning ratios on LongBench.}\vspace{4pt}\label{tab:pruningkv}
\scalebox{0.6}{\begin{tabular}{l|lcccccccccccccccccc}
    \toprule
&\multirow{4}{*}{Method}& \multirow{4}{*}{$\lambda$}& \multicolumn{3}{c}{Single-Document QA} & \multicolumn{3}{c}{Multi-Document QA}& \multicolumn{3}{c}{Summarization}& \multicolumn{3}{c}{Few-shot Learning}& \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{Code}&\multirow{4}{*}{Avg.} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}
&&& \rotatebox[origin=c]{30}{NrtvQA} & \rotatebox[origin=c]{30}{Qasper} & \rotatebox[origin=c]{30}{MF-en} & \rotatebox[origin=c]{30}{HotpotQA} & \rotatebox[origin=c]{30}{2WikiMQA} & \rotatebox[origin=c]{30}{Musique} & \rotatebox[origin=c]{30}{GovReport} & \rotatebox[origin=c]{30}{QMSum} & \rotatebox[origin=c]{30}{MultiNews} & \rotatebox[origin=c]{30}{TREC} & \rotatebox[origin=c]{30}{TriviaQA} & \rotatebox[origin=c]{30}{SAMSum} & \rotatebox[origin=c]{30}{PCount} & \rotatebox[origin=c]{30}{PRe} & \rotatebox[origin=c]{30}{Lcc} & \rotatebox[origin=c]{30}{RB-P} \\
&\multicolumn{19}{c}{KV-size Full}\\
\multirow{13}{*}{\rotatebox[origin=c]{90}{ Mistral 7B}}

    & ALL KV & 0  & 26.63 & 32.99 & 49.34 & 42.77 & 27.35 & 18.77 & 32.87 & 24.24 & 27.1 & 71.0 & 86.23 & 42.96 & 2.75 & 86.98 & 56.93 & 54.49 & 42.71\\
\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 128}\\
    & H2O      & 0  &  21.21 & 21.81 & 38.87 & 30.42 & 20.36 & 12.30 & 20.58 & 22.61 & 22.10 & 39.00 & 82.37 & 40.44 & 2.90 & 79.56 & 51.22 & 48.38 & 34.63 \\
    & H2O(99)  & 0  & 20.87 & 21.38 & 37.52 & 29.31 & 21.28 & 13.46 & 19.78 & 22.38 & 20.94 & 38.00 & 82.61 & 39.36 & 3.69 & 77.11 & 50.53 & 48.18 & 34.15 \\
    & H2O(109)  & 0  & 21.29 & 20.69 & 37.66 & 28.65 & 21.08 & 14.01 & 20.20 & 22.11 & 21.33 & 38.50 & 82.55 & 39.87 & 3.66 & 78.14 & 50.32 & 48.54 & 34.29 \\
    & H2O+\our(l2) & 30+30 & 21.36 & 19.39 & 38.27 & 29.55 & 22.14 & 12.79 & 19.89 & 21.85 & 21.04 & 37.50 & 81.38 & 38.44 & 2.91 & 71.89 & 51.07 & 47.66 & 33.57 \\
    & H2O+\our(l2) & 20+20 & 21.09 & 21.11 & 39.00 & 30.36 & 21.93 & 14.05 & 20.18 & 22.20 & 21.26 & 38.00 & 82.17 & 39.66 & 3.57 & 77.28 & 51.39 & 48.84 & 34.51 \\
    & H2O+\our(new) & 30+30 & 21.51 & 21.05 & 39.19 & 30.25 & 21.71 & 12.81 & 20.41 & 22.38 & 21.3 & 37.5 & 81.95 & 38.98 & 3.36 & 73.29 & 51.52 & 48.68 & 34.12\\
    & H2O+\our(new2) & 30+30 & 20.71 & 21.49 & 38.01 & 30.66 & 22.28 & 13.87 & 20.13 & 22.45 & 21.07 & 38.5 & 82.2 & 38.69 & 2.94 & 78.56 & 51.55 & 48.28 & 34.46 \\
    & H2O+\our(new2) & 40+0 & 21.17 & 21.9 & 39.29 & 29.92 & 20.99 & 12.30 & 20.84 & 22.91 & 21.92 & 39.00 & 82.70 & 40.35 & 2.97 & 79.21 & 51.19 & 48.32 & 34.69 \\
    & H2O+\our(new2) & 50+0 & 21.67 & 21.8 & 39.48 & 28.74 & 20.65 & 13.14 & 20.57 & 22.83 & 21.78 & 39.0 & 82.54 & 40.12 & 3.61 & 78.39 & 50.27 & 48.4 &34.56 \\
    & H2O+\our(new2) & 60+0 & 21.04 & 21.3 & 39.56 & 28.68 & 21.29 & 13.97 & 20.13 & 22.52 & 21.81 & 39.5 & 82.05 & 39.14 & 4.16 & 74.23 & 49.83 & 47.67 & 34.18 \\
    \cdashline{2-20}    
    & SnapKV      & 0  & 19.17 & 21.4 & 42.93 & 36.76 & 22.44 & 15.86 & 19.16 & 21.84 & 21.55 & 47.50 & 84.15 & 40.24 & 2.30 & 68.26 & 52.31 & 48.80 & 35.29 \\
    & SnapKV(99)  & 0  & 18.80 & 19.01 & 42.81 & 37.82 & 22.28 & 15.20 & 18.30 & 21.37 & 20.37 & 44.00 & 83.56 & 39.24 & 3.10 & 62.4 & 50.59 & 47.03 & 34.12 \\
    & SnapKV(109)  & 0  & 19.25 & 19.95 & 42.8 & 35.88 & 21.96 & 14.59 & 18.76 & 21.71 & 20.70 & 46.00 & 84.12 & 39.43 & 2.59 & 65.36 & 51.39 & 47.81 & 34.52 \\
    & SnapKV+\our(l2) & 30+30 & 21.39 & 19.72 & 42.85 & 36.78 & 21.41 & 14.68 & 18.61 & 21.76 & 20.76 & 42.00 & 82.89 & 39.12 & 3.43 & 61.46 & 51.52 & 47.89 & 34.14 \\
    & SnapKV+\our(l2) & 20+20 & 20.79 & 19.94 & 43.42 & 36.05 & 21.97 & 14.57 & 19.22 & 21.68 & 20.75 & 45.50 & 82.71 & 39.84 & 3.57 & 61.92 & 52.06 & 48.41 & 34.53 \\
    & SnapKV+\our(new) & 30+30 & 21.85 & 20.03 & 43.97 & 39.23 & 22.67 & 14.88 & 19.27 & 22.17 & 20.99 & 44.50 & 83.52 & 39.14 & 3.56 & 62.88 & 52.16 & 49.09 & 34.99 \\
    & SnapKV+\our(new2) & 30+30 & 19.92 & 20.61 & 42.68 & 37.63 & 23.19 & 15.09 & 18.97 & 21.93 & 20.55 & 45.00 & 84.06 & 39.33 & 2.99 & 66.00 & 51.51 & 47.51 & 34.81 \\
    & SnapKV+\our(new2) & 40+0 & 20.52 & 21.00 & 42.65 & 37.58 & 22.09 & 15.23 & 19.29 & 22.01 & 21.22 & 47.00 & 83.85 & 39.64 & 3.20 & 67.45 & 51.48 & 48.31 & 35.16 \\
    & SnapKV+\our(new2) & 50+0 & 20.67 & 20.6 & 43.37 & 37.27 & 21.58 & 15.66 & 19.06 & 21.79 & 21.02 & 47.0 & 83.38 & 39.77 & 3.65 & 67.06 & 50.8 & 48.35 & 35.06 \\
    & SnapKV+\our(new2) & 60+0 & 21.25 & 20.82 & 44.2 & 36.21 & 21.68 & 16.47 & 19.05 & 21.99 & 20.73 & 45.0 & 83.81 & 38.79 & 4.19 & 66.9 & 49.99 & 47.61 & 34.92 \\

\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 512}\\

    
    & H2O      & 0  &  21.83 & 26.00 & 44.69 & 32.46 & 23.05 & 14.69 & 23.53 & 23.06 & 24.59 & 42.00 & 85.22 & 41.49 & 3.40 & 86.20 & 54.78 & 51.09 & 37.38 \\
    & H2O(435)  & 0  & 22.42 & 24.13 & 43.26 & 31.02 & 23.57 & 13.78 & 23.38 & 22.90 & 23.82 & 42.00 & 85.04 & 41.47 & 3.00 & 86.45 & 54.72 & 50.73 & 36.98 \\
    & H2O(400)  & 0  & 21.93 & 24.12 & 43.24 & 30.73 & 23.42 & 13.90 & 23.02 & 23.26 & 24.10 & 41.00 & 84.46 & 41.02 & 3.040 & 86.03 & 54.50 & 50.36 & 36.76 \\
    & H2O+\our(l2) & 20+20 & 22.48 & 24.52 & 44.18 & 31.02 & 23.21 & 14.97 & 22.91 & 23.34 & 24.38 & 40.50 & 85.69 & 41.64 & 2.96 & 78.57 & 54.01 & 50.49 & 36.55 \\
    & H2O+\our(new) & 30+0 & 21.58 & 25.65 & 44.72 & 33.12 & 23.33 & 15.01 & 23.88 & 22.89 & 24.69 & 42.0 & 85.57 & 41.67 & 2.98 & 86.15 & 54.46 & 51.41 & 37.44 \\
    & H2O+\our(new2) & 30+30  & 22.36 & 24.26 & 44.77 & 30.47 & 22.94 & 14.96 & 22.63 & 22.90 & 23.73 & 41.50 & 85.30 & 40.21 & 3.08 & 80.07 & 54.48 & 50.96 & 36.54 \\
    & H2O+\our(new2) & 30+20  & 22.42 & 25.73 & 44.72 & 31.31 & 23.10 & 14.02 & 22.86 & 22.85 & 23.99 & 41.50 & 85.63 & 41.51 & 2.51 & 82.92 & 54.93 & 51.30 & 36.96 \\
    & H2O+\our(new2) & 30+10  & 22.14 & 25.15 & 45.29 & 31.78 & 23.21 & 14.62 & 23.36 & 22.70 & 24.51 & 41.50 & 85.61 & 41.58 & 2.75 & 84.03 & 54.50 & 51.09 & 37.11 \\
    & H2O+\our(new2) & 40+0  & 22.07 & 25.85 & 44.64 & 32.02 & 23.74 & 15.18 & 23.72 & 23.43 & 24.34 & 42.00 & 85.58 & 42.47 & 3.25 & 85.70 & 54.38 & 51.11 & 37.47 \\
    & H2O+\our(new2) & 50+0  & 22.49 & 26.01 & 44.19 & 31.7 & 22.97 & 14.72 & 23.57 & 22.56 & 24.34 & 41.5 & 85.7 & 41.58 & 2.82 & 84.57 & 54.89 & 50.68 & 37.14 \\
    & H2O+\our(new2) & 60+0  & 22.91 & 25.57 & 44.04 & 29.48 & 22.88 & 13.67 & 23.31 & 22.64 & 24.1 & 41.0 & 85.31 & 41.15 & 2.98 & 82.34 & 53.7 & 50.25 & 36.58 \\
    \cdashline{2-20}
    & SnapKV      & 0  &  24.44 & 27.81 & 48.98 & 39.46 & 25.25 & 16.98 & 23.70 & 22.96 & 24.37 & 67.0 & 85.88 & 41.26 & 2.78 & 86.56 & 56.46 & 53.41 & 40.46 \\
    & SnapKV(435)  & 0  & 24.05 & 27.41 & 48.70 & 38.75 & 24.24 & 16.36 & 23.43 & 23.15 & 24.33 & 66.50 & 86.00 & 40.95 & 2.72 & 87.93 & 56.15 & 52.92 & 40.22 \\
    & SnapKV(400)  & 0  & 23.49 & 26.57 & 48.80 & 38.55 & 23.92 & 16.39 & 23.19 & 23.13 & 23.91 & 66.00 & 85.69 & 41.11 & 2.52 & 87.99 & 55.87 & 53.02 & 40.01 \\
    & SnapKV+\our(l2) & 20+20 & 25.00 & 27.81 & 48.15 & 38.5 & 25.45 & 16.12 & 22.82 & 23.16 & 24.19 & 66.5 & 86.38 & 40.94 & 3.88 & 82.63 & 56.25 & 52.68 & 40.03 \\
    & SnapKV+\our(new) & 30+30 & 24.86 & 27.73 & 47.69 & 38.69 & 25.15 & 17.25 & 22.86 & 22.83 & 23.94 & 66.50 & 86.55 & 40.52 & 2.72 & 76.14 & 56.03 & 52.97 & 39.53 \\
    & SnapKV+\our(new2) & 30+30 & 24.10 & 27.04 & 47.76 & 38.66 & 25.45 & 17.51 & 22.64 & 22.81 & 23.91 & 66.00 & 86.62 & 39.91 & 3.36 & 82.24 & 55.96 & 52.81 & 39.80 \\
    & SnapKV+\our(new2) & 30+10 & 23.90 & 28.14 & 48.35 & 39.03 & 24.83 & 16.68 & 23.51 & 23.12 & 24.34 & 67.50 & 86.09 & 41.69 & 2.65 & 84.34 & 57.29 & 53.22 & 40.29 \\
    & SnapKV+\our(new2) & 40+0 & 24.32 & 28.62 & 48.97 & 38.55 & 24.82 & 16.80 & 23.51 & 23.40 & 24.53 & 67.50 & 85.90 & 42.25 & 3.08 & 85.45 & 55.91 & 53.39 & 40.44 \\
    & SnapKV+\our(new2) & 50+0 & 24.56 & 29.22 & 48.59 & 37.7 & 24.27 & 17.39 & 23.68 & 23.65 & 24.58 & 67.5 & 86.05 & 42.01 & 3.07 & 86.3 & 56.49 & 53.29 & 40.52 \\
    & SnapKV+\our(new2) & 60+0 & 24.38 & 28.25 & 48.82 & 38.61 & 24.26 & 17.14 & 23.47 & 23.41 & 24.26 & 67.0 & 86.32 & 40.12 & 3.62 & 84.45 & 55.32 & 52.38 & 40.11 \\
    
\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 1024}\\

    
    & H2O      & 0  &  23.67 & 28.55 & 46.4 & 36.99 & 24.82 & 15.02 & 25.21 & 23.04 & 25.77 & 46.00 & 85.93 & 41.98 & 3.24 & 86.57 & 56.40 & 52.75 & 38.90 \\
    & H2O+\our(new) & 30+30 & 24.33 & 26.86 & 46.68 & 36.15 & 25.13 & 15.77 & 24.21 & 23.44 & 25.11 & 44.50 & 86.56 & 41.42 & 2.99 & 73.70 & 55.90 & 52.29 & 37.82 \\
    & H2O+\our(new2) & 30+30 & 23.65 & 26.54 & 47.00 & 35.52 & 24.79 & 17.15 & 23.64 & 23.12 & 25.20 & 44.00 & 86.38 & 41.67 & 3.46 & 80.14 & 56.53 & 52.86 & 38.23 \\
    & H2O+\our(new2) & 30+10 & 24.13 & 28.57 & 46.31 & 35.59 & 24.92 & 15.34 & 24.58 & 23.33 & 25.93 & 45.50 & 85.91 & 42.97 & 2.57 & 83.64 & 55.39 & 52.73 & 38.59 \\
    & H2O+\our(new2) & 40+0 & 23.94 & 29.08 & 45.84 & 35.93 & 24.89 & 14.51 & 25.15 & 23.27 & 26.15 & 45.00 & 86.11 & 42.57 & 3.23 & 84.82 & 56.02 & 52.85 & 38.71 \\
    & H2O+\our(new2) & 50+0 & 24.16 & 28.52 & 46.47 & 35.61 & 24.17 & 14.72 & 24.84 & 23.28 & 25.87 & 44.5 & 86.15 & 42.69 & 3.34 & 83.2 & 56.1 & 52.68 & 38.52 \\
    & H2O+\our(new2) & 60+0 & 23.65 & 28.21 & 46.52 & 36.03 & 24.96 & 14.92 & 24.18 & 23.45 & 25.41 & 44.5 & 85.05 & 42.04 & 3.34 & 81.92 & 55.17 & 51.93 & 38.21 \\
    % & H2O(845)  & 0  & 22.74 & 28.10 & 46.03 & 35.56 & 24.06 & 13.95 & 24.76 & 22.98 & 25.68 & 45.50 & 85.54 & 41.62 & 3.02 & 85.82 & 56.11 & 52.33 & 38.36 \\
    % & H2O+\our(l2) & 20+20 & 24.04 & 27.46 & 45.69 & 35.5 & 25.53 & 14.83 & 24.2 & 23.26 & 25.32 & 42.5 & 86.94 & 41.94 & 2.92 & 79.77 & 56.0 & 52.83 & 38.05 \\
    \cdashline{2-20}    
    & SnapKV      & 0  & 25.47 & 29.57 & 49.33 & 40.90 & 25.53 & 19.01 & 25.94 & 23.89 & 26.21 & 69.50 & 86.48 & 42.10 & 2.98 & 88.56 & 57.19 & 53.60 & 41.64 \\
    & SnapKV+\our(new) & 30+30 & 25.65 & 28.04 & 48.63 & 40.56 & 25.09 & 18.22 & 24.23 & 23.41 & 25.17 & 68.5 & 87.01 & 41.0 & 3.16 & 77.01 & 56.7 & 54.21 & 40.41 \\
    & SnapKV+\our(new2) & 30+30 & 25.29 & 29.25 & 49.17 & 41.25 & 25.75 & 19.37 & 24.64 & 23.02 & 25.27 & 69.00 & 86.70 & 40.92 & 3.29 & 82.06 & 57.15 & 54.15 & 41.02 \\
    & SnapKV+\our(new2) & 30+10 & 25.84 & 29.30 & 49.56 & 41.44 & 25.29 & 19.02 & 25.21 & 23.73 & 25.72 & 69.00 & 86.69 & 42.55 & 2.44 & 85.76 & 57.55 & 54.10 & 41.45 \\
    & SnapKV+\our(new2) & 40+0 & 25.22 & 30.48 & 48.58 & 41.11 & 25.28 & 18.99 & 25.91 & 24.00 & 26.13 & 70.00 & 86.64 & 43.35 & 2.98 & 86.3 & 56.71 & 54.19 & 41.62 \\
    & SnapKV+\our(new2) & 50+0 & 25.71 & 30.26 & 49.5 & 40.78 & 25.1 & 19.1 & 25.48 & 23.86 & 25.94 & 69.5 & 86.92 & 42.13 & 2.82 & 84.73 & 57.34 & 53.72 & 41.43 \\
    & SnapKV+\our(new2) & 60+0 & 25.44 & 29.06 & 49.11 & 40.52 & 25.23 & 19.52 & 25.3 & 23.82 & 25.82 & 69.0 & 86.85 & 40.93 & 3.07 & 83.36 & 56.56 & 53.31 & 41.06 \\
    % & SnapKV(845)  & 0  & 24.44 & 29.31 & 49.52 & 40.72 & 24.91 & 18.69 & 25.41 & 23.77 & 25.76 & 68.5 & 86.31 & 41.61 & 3.15 & 88.05 & 57.2 & 53.83 & 41.32 \\
    % & SnapKV+\our(l2) & 20+20 & 24.57 & 29.50 & 49.26 & 40.13 & 26.37 & 18.31 & 24.34 & 24.08 & 25.51 & 68.50 & 87.19 & 42.14 & 3.38 & 82.45 & 57.33 & 53.99 & 41.07 \\
\cmidrule{2-20}
&\multicolumn{19}{c}{KV-size 2048}\\

    
    & H2O      & 0  &  25.76 & 31.10 & 49.06 & 40.38 & 26.43 & 16.78 & 27.17 & 23.64 & 26.69 & 55.0 & 86.35 & 42.48 & 2.72 & 86.64 & 56.98 & 53.91 & 40.69\\
    & H2O(1480)  & 0  & 25.29 & 30.24 & 46.91 & 39.09 & 25.31 & 16.13 & 26.78 & 23.39 & 26.60 & 50.00 & 86.48 & 42.16 & 3.21 & 85.07 & 56.98 & 53.59 & 39.83 \\
    & H2O+\our(new) & 30+30 & 25.56 & 29.58 & 47.62 & 40.53 & 26.25 & 17.42 & 25.23 & 23.12 & 26.08 & 52.00 & 86.72 & 42.55 & 2.81 & 76.96 & 56.88 & 54.09 & 39.59 \\
    & H2O+\our(new2) & 30+30  & 25.60 & 28.74 & 47.54 & 38.67 & 26.25 & 17.35 & 24.54 & 23.27 & 26.15 & 51.00 & 87.01 & 43.02 & 2.94 & 81.46 & 56.41 & 54.26 & 39.64 \\
    & H2O+\our(new2) & 30+10  & 25.64 & 30.65 & 48.95 & 40.42 & 26.43 & 16.65 & 26.76 & 23.51 & 26.59 & 52.50 & 86.53 & 43.45 & 2.66 & 83.96 & 56.55 & 53.83 & 40.32 \\
    & H2O+\our(new2) & 40+0  & 25.69 & 30.93 & 48.32 & 39.63 & 26.08 & 16.82 & 27.18 & 23.92 & 26.62 & 53.50 & 86.39 & 42.96 & 3.29 & 86.39 & 56.77 & 53.6 & 40.51 \\
    & H2O+\our(new2) & 50+0  & 25.68 & 31.24 & 48.69 & 39.65 & 25.84 & 16.72 & 26.69 & 23.57 & 26.78 & 52.0 & 86.74 & 42.85 & 4.01 & 83.46 & 57.12 & 53.67 & 40.29 \\
    & H2O+\our(new2) & 60+0  & 25.97 & 31.02 & 48.51 & 38.56 & 26.2 & 16.57 & 26.7 & 23.99 & 26.19 & 51.0 & 86.36 & 42.09 & 3.52 & 82.49 & 56.03 & 52.76 & 39.87 \\
    \cdashline{2-20}    
    & SnapKV      & 0  & 25.89 & 32.56 & 48.55 & 41.68 & 27.24 & 18.75 & 28.90 & 24.47 & 26.63 & 70.00 & 86.27 & 42.57 & 3.09 & 86.93 & 57.44 & 53.83 & 42.18 \\
    & SnapKV(1480)  & 0  & 25.27 & 31.67 & 48.08 & 41.08 & 26.39 & 19.23 & 27.39 & 23.99 & 26.32 & 70.00 & 86.32 & 42.50 & 3.16 & 88.18 & 56.68 & 53.92 & 41.89 \\
    & SnapKV+\our(new) & 30+30 & 26.69 & 31.88 & 48.69 & 40.94 & 27.12 & 17.78 & 26.41 & 23.49 & 26.14 & 70.00 & 86.92 & 40.74 & 2.88 & 76.95 & 57.02 & 54.46 & 41.13 \\
    & SnapKV+\our(new2) & 30+30 & 27.01 & 30.72 & 48.81 & 41.15 & 26.93 & 18.93 & 25.81 & 23.59 & 26.42 & 70.00 & 86.82 & 41.91 & 3.05 & 82.65 & 57.01 & 54.25 & 41.57 \\
    & SnapKV+\our(new2) & 30+10 & 26.22 & 32.69 & 48.96 & 40.83 & 26.70 & 19.02 & 27.87 & 24.23 & 26.64 & 70.00 & 86.65 & 42.63 & 2.22 & 85.13 & 57.00 & 54.28 & 41.94 \\
    & SnapKV+\our(new2) & 40+0 & 25.75 & 32.49 & 48.61 & 41.01 & 27.18 & 19.14 & 28.79 & 24.64 & 26.77 & 70.00 & 86.37 & 42.77 & 3.61 & 87.13 & 57.19 & 54.39 & 42.24 \\
    & SnapKV+\our(new2) & 50+0 & 26.49 & 32.73 & 48.99 & 40.82 & 27.32 & 19.58 & 28.36 & 24.26 & 26.84 & 70.0 & 86.5 & 41.68 & 2.78 & 84.7 & 56.55 & 53.98 & 41.97 \\
    & SnapKV+\our(new2) & 60+0 & 26.14 & 32.47 & 49.06 & 40.86 & 27.22 & 19.04 & 27.95 & 23.99 & 26.52 & 70.0 & 86.45 & 41.4 & 3.34 & 82.34 & 56.09 & 53.39 & 41.64 \\
    \bottomrule
    \end{tabular}}
    \end{table}



==> tables/think_llama70.tex <==
\begin{table}[t!]
    \centering \scriptsize
    \caption{Performance comparison of key cache pruning on LLaMA3-70B by ThinK on LongBench.}\vspace{4pt}\label{tab:think_llama70}
\resizebox{\textwidth}{!}{\begin{tabular}
% {lcccccccccccccccccc}
{l@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.05ex}}c@{\hspace{0.6ex}}c@{\hspace{0.6ex}}c@{\hspace{0.6ex}}c@{\hspace{0.6ex}}c}
    \toprule
\multirow{4}{*}{Method}& \multicolumn{3}{c}{Single-Document QA} & \multicolumn{3}{c}{Multi-Document QA}& \multicolumn{3}{c}{Summarization}& \multicolumn{3}{c}{Few-shot Learning}& \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{Code}&\multirow{4}{*}{Avg.} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
& \rotatebox[origin=c]{30}{NrtvQA} & \rotatebox[origin=c]{30}{Qasper} & \rotatebox[origin=c]{30}{MF-en} & \rotatebox[origin=c]{30}{HotpotQA} & \rotatebox[origin=c]{30}{2WikiMQA} & \rotatebox[origin=c]{30}{Musique} & \rotatebox[origin=c]{30}{GovReport} & \rotatebox[origin=c]{30}{QMSum} & \rotatebox[origin=c]{30}{MultiNews} & \rotatebox[origin=c]{30}{TREC} & \rotatebox[origin=c]{30}{TriviaQA} & \rotatebox[origin=c]{30}{SAMSum} & \rotatebox[origin=c]{30}{PCount} & \rotatebox[origin=c]{30}{~PRe~~} & \rotatebox[origin=c]{30}{~Lcc~~} & \rotatebox[origin=c]{30}{~RB-P~} \\
\cmidrule{1-18}
\multicolumn{18}{c}{KV-size 128}\\ 
    SnapKV & 25.91 & 39.41 & 43.83 & 49.60 & 51.23 & 27.76 & 22.14 & 21.91 & 23.16 & 69.00 & 91.55 & 43.54 & 12.50 & 72.00 & 48.41 & 63.49 & 44.09 \\
     +\our(0.4)  & 25.64 & 39.20 & 43.60 & 50.22 & 50.50 & 29.32 & 21.70 & 21.96 & 23.35 & 68.00 & 91.27 & 43.24 & 12.50 & 73.00 & 48.01 & 62.43 & 44.00 \\
     +\our(0.5)   & 26.31 & 38.76 & 44.86 & 48.54 & 49.62 & 28.97 & 21.46 & 22.01 & 22.91 & 67.00 & 91.52 & 43.15 & 12.50 & 72.50 & 47.21 & 60.82 & 43.63 \\
\cmidrule{1-18}
\multicolumn{18}{c}{KV-size 512}\\ 
    SnapKV & 27.95 & 45.19 & 48.50 & 50.97 & 54.53 & 29.78 & 25.34 & 22.36 & 26.03 & 73.50 & 92.63 & 45.07 & 12.50 & 72.50 & 45.21 & 68.22 & 46.27 \\
     +\our(0.4)  & 27.47 & 45.31 & 48.57 & 51.22 & 54.32 & 30.05 & 25.42 & 22.72 & 26.20 & 73.50 & 92.13 & 45.53 & 12.50 & 73.00 & 48.32 & 66.99 & 46.45 \\
     +\our(0.5)   & 26.97 & 44.55 & 48.16 & 50.84 & 53.80 & 30.57 & 25.29 & 22.65 & 25.53 & 73.00 & 92.13 & 43.66 & 12.50 & 73.00 & 50.52 & 64.82 & 46.12 \\
\cmidrule{1-18}
\multicolumn{18}{c}{KV-size 1024}\\ 
    SnapKV & 26.80 & 46.21 & 49.93 & 51.70 & 54.71 & 29.86 & 27.61 & 22.43 & 27.15 & 73.50 & 92.38 & 46.18 & 12.50 & 72.50 & 42.84 & 69.89  & 46.64 \\
     +\our(0.4)  & 27.04 & 46.01 & 50.13 & 51.96 & 54.36 & 29.87 & 27.74 & 22.78 & 27.07 & 73.50 & 91.88 & 46.35 & 12.50 & 73.00 & 45.05 & 67.87 & 46.69 \\
     +\our(0.5)   & 27.62 & 46.22 & 48.97 & 51.79 & 53.39 & 30.47 & 27.45 & 23.05 & 26.57 & 73.50 & 91.88 & 43.99 & 12.50 & 72.50 & 47.41 & 66.84 & 46.51 \\
\cmidrule{1-18}     
\multicolumn{18}{c}{KV-size 2048}\\ 
    SnapKV & 27.44 & 46.51 & 49.60 & 51.80 & 54.77 & 31.05 & 29.67 & 22.44 & 27.43 & 73.50 & 92.38 & 45.98 & 12.50 & 72.50 & 41.86 & 68.72 & 46.76 \\
     +\our(0.4)  & 27.13 & 46.26 & 50.04 & 51.72 & 55.03 & 31.19 & 29.75 & 22.47 & 27.28 & 73.50 & 91.88 & 46.37 & 12.50 & 72.50 & 42.66 & 67.77 & 46.75 \\
     +\our(0.5)   & 27.84 & 46.86 & 49.18 & 51.97 & 53.58 & 31.44 & 29.41 & 22.89 & 27.33 & 73.50 & 91.88 & 43.60 & 12.50 & 72.50 & 44.78 & 66.65 & 46.62 \\


    \bottomrule
    \end{tabular}}
    \end{table}


==> tables/v-pruning.tex <==
\begin{table}[htp]
    \centering \scriptsize
    \caption{Performance comparison of pruning V cache with different pruning ratios on LongBench.}\vspace{4pt}\label{tab:pruningv}
\scalebox{0.6}{\begin{tabular}{l|lcccccccccccccccccc}
    \toprule
&\multirow{4}{*}{~~~Method}& \multirow{4}{*}{$\gamma$}& \multicolumn{3}{c}{Single-Document QA} & \multicolumn{3}{c}{Multi-Document QA}& \multicolumn{3}{c}{Summarization}& \multicolumn{3}{c}{Few-shot Learning}& \multicolumn{2}{c}{Synthetic} & \multicolumn{2}{c}{Code}&\multirow{4}{*}{Avg.} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}
&&& \rotatebox[origin=c]{30}{NrtvQA} & \rotatebox[origin=c]{30}{Qasper} & \rotatebox[origin=c]{30}{MF-en} & \rotatebox[origin=c]{30}{HotpotQA} & \rotatebox[origin=c]{30}{2WikiMQA} & \rotatebox[origin=c]{30}{Musique} & \rotatebox[origin=c]{30}{GovReport} & \rotatebox[origin=c]{30}{QMSum} & \rotatebox[origin=c]{30}{MultiNews} & \rotatebox[origin=c]{30}{TREC} & \rotatebox[origin=c]{30}{TriviaQA} & \rotatebox[origin=c]{30}{SAMSum} & \rotatebox[origin=c]{30}{PCount} & \rotatebox[origin=c]{30}{PRe} & \rotatebox[origin=c]{30}{Lcc} & \rotatebox[origin=c]{30}{RB-P} \\
\multirow{9}{*}{\rotatebox[origin=c]{90}{ LLaMA3 8B}}

    & ALL KV & 0  &25.70 &29.75 &41.12 &45.55 &35.87 &22.35 &25.63 &23.03 &26.21 &73.00 &90.56 &41.88 &4.67 &69.25 &58.05 &50.77 &41.46 \\
\cmidrule(lr){2-20}
    & H2O         & 0   & 23.52 & 17.93 & 34.68 & 42.11 & 33.52 & 19.92 & 22.11 & 22.56 & 23.82 & 41.00 & 90.46 & 40.20 & 5.87 & 69.50 & 56.71 & 51.69 & 37.23 \\
    & H2O+\our(l1)    & 30  & 23.93 & 18.66 & 35.69 & 42.09 & 36.56 & 21.38 & 21.55 & 21.98 & 23.38 & 38.50 & 89.62 & 39.69 & 6.04 & 69.50 & 56.94 & 50.97 & 37.28 \\
    & H2O+\our(l1)    & 40  & 22.76 & 17.97 & 35.80 & 42.77 & 35.98 & 21.83 & 20.98 & 21.94 & 22.98 & 38.00 & 89.49 & 38.83 & 6.13 & 69.50 & 57.17 & 51.27 & 37.09 \\
    & H2O+\our(l1)    & 50  & 23.22 & 18.06 & 35.62 & 43.19 & 34.36 & 21.56 & 20.51 & 22.28 & 22.14 & 38.00 & 89.48 & 38.07 & 5.88 & 69.50 & 56.83 & 51.39 & 36.88 \\

\cmidrule(lr){2-20}
    & SnapKV      & 0  & 24.84 & 23.96 & 38.77 & 42.75 & 34.55 & 20.87 & 22.26 & 22.61 & 23.97 & 70.00 & 90.52 & 40.29 & 5.81 & 69.50 & 59.04 & 51.81 & 40.10 \\
    & SnapKV+\our(l1) & 30 & 24.24 & 25.48 & 37.98 & 44.20 & 36.56 & 21.22 & 21.48 & 22.37 & 23.67 & 67.00 & 90.33 & 39.53 & 5.79 & 69.50 & 59.21 & 52.92 & 40.09 \\
    & SnapKV+\our(l1) & 40 & 23.77 & 25.58 & 37.32 & 44.62 & 36.57 & 21.36 & 21.08 & 22.41 & 23.24 & 65.50 & 90.39 & 38.74 & 5.92 & 69.17 & 58.68 & 53.55 & 39.87 \\
    & SnapKV+\our(l1) & 50 & 23.91 & 25.55 & 37.33 & 44.15 & 35.92 & 22.31 & 20.79 & 22.15 & 22.83 & 65.00 & 90.75 & 38.02 & 6.08 & 69.50 & 58.37 & 53.50 & 39.76 \\
    %& - & 44.8 & 35.7 & \textcolor{red}{3537 chars} & 69.3 & 39.0 & 58.2\\
    %Ours-Mix2 & 0.001 & 41.9  & 22.1 & 382 & 78.8 & 66.5 & 62.4 \\
    %Ours-Mix2 & No & 37.2  & 29.1 & 656 & - & 64.6 & 60.8\\
    \bottomrule
    \end{tabular}}
    \end{table}

